Sandi: A System for Accountability

We present a system, Sandi, for creating trust through accountability. Concretely, we focus on online communication scenarios, where the communicating parties do not know each other, yet would benefit from a degree of initial trust. Sandi can be seen as a reputation system that measures bad behavior, with strong integrity protections and resistance to manipulation. Unlike most reputation systems, Sandi is entirely based on ``downvotes'' and therefore requires strong privacy guarantees to prevent retaliation. It utilizes a ticket-based reporting mechanism to limit who can report. We also prove that Sandi incentivizes good behavior in a well-defined sense. Sandi is by design unidirectional, so that message senders have Sandi scores and receivers can report them for inappropriate communication, but it is designed to benefit both senders and receivers. Senders benefit, as receivers are more likely to react to communication with the added trust signal. Receivers benefit from seeing senders' scores, allowing them to make more informed decisions about which senders to trust. Receivers do not need registered accounts and neither senders nor receivers need long-term keys. Sandi guarantees score integrity, communication privacy, reporter privacy to protect reporting receivers, and sender unlinkability. Sandi can be implemented on top of any communication system that allows for small binary data transfer.

==> ethics.tex <==
\section{Ethics Considerations}
We have introduced a reputation system design that provides a measure of reputation with strong security and privacy properties and a formal optimality analysis.
Taken together, these features imply a form of resistance to manipulation, meaning that adversarial parties cannot easily make the system deviate too much from its intended behavior, at least without the manipulation being detected.
While our primary focus was on applying \oursystem to communication systems, its abstract design necessitates an ethical analysis covering other use-cases as well.
We approach this through the lenses of consequentialist and deontological ethics.

Reputation systems are widely deployed across the Internet to assist individuals in decision-making, and in many cases these systems play an outsized role in protecting the most vulnerable populations from bad outcomes.
It seems therefore fair to say that reputation systems, as deployed already today, have significant societal benefits.
From a consequentialist utilitarian perspective, reducing their vulnerability to manipulation may improve their effectiveness in delivering accurate and trustworthy signals, thereby maximizing their utility and benefit to society as a whole. 
That's the core of our design goals.

A consequentialist analysis must also consider the unintended consequences of privacy-preserving reputation systems.
Namely, privacy and security properties can inadvertently shield abusive behavior, complicating detection and mitigation.
Endorsement tags (a form of ``ticket'' for submitting a report) and the tolerance level \bonus were put in place to mitigate this risk of colluding receivers maliciously targeting (``badmouthing'') a sender.
The sender's unlinkability guarantee was designed to protect the sender, but can also be used to prevent a receiver from realizing it is interacting with a single (potentially malicious) entity.
While the sender's capability for doing this is limited for the benefit of reporter privacy (\autoref{sec:anonymous_reporting}), there can still be potential for abusive use.

Reputation systems have a long history of being used by authoritarian regimes for monitoring their citizens.
Indeed, even the simplest reputation systems pose ethical dilemmas under authoritarian control.
One should ask if and how the privacy and security features we present contribute to such use.
We argue that they do not, because such a regime running \accountabilityServer has no reason to provide score integrity guarantees and can be thought of as effectively colluding with (a subset of) their citizens to target and report others.
This makes our privacy and security guarantees meaningless.


In conclusion, from a utilitarian perspective, the benefits of reliable reputation systems can be substantial.
Even though most, if not all, reputation systems can be deployed for malicious purposes, creating systems with stronger privacy, security, and accountability controls can mitigate potential harms while maximizing societal benefit on a global scale.

From a deontological perspective, digital platform and service providers have a moral duty to protect the privacy and security of their users, respecting individuals' rights to autonomy and privacy.
Privacy technologies, such as the ones developed in this work, support these rights by minimizing the providers' access to data and unnecessary control of the system, ensuring individuals are treated as ends in themselves rather than merely as means.
Moreover, reducing manipulation promotes fairness and equality for all users.

